Collapsed Language Models Promote Fairness

To mitigate societal biases implicitly encoded in recent successful pretrained language models, a diverse array of approaches have been proposed to encourage model fairness, focusing on prompting, data augmentation, regularized fine-tuning, and more. Despite the development, it is nontrivial to reach a principled understanding of fairness and an effective algorithm that can consistently debias language models. In this work, by rigorous evaluations of Neural Collapse -- a learning phenomenon happen in last-layer representations and classifiers in deep networks -- on fairness-related words, we find that debiased language models exhibit collapsed alignment between token representations and word embeddings. More importantly, this observation inspires us to design a principled fine-tuning method that can effectively improve fairness in a wide range of debiasing methods, while still preserving the performance of language models on standard natural language understanding tasks. We attach our code at https://github.com/Xujxyang/Fairness-NC-main.

==> Table/parallel.tex <==
\begin{table}[!t]
    \centering
    \begin{minipage}[b]{0.51\textwidth}
        \centering
        \caption{Fine-tuning results on Bias-in-Bios.}
        % \jingxuan{I believe the original is correct; they are all TPR scores}
        \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{lcccccl} \toprule
            &  {Acc.}  & {Acc.} & {Acc.} & \textbf{TPR} & \textbf{TPR} \\ 
            \textbf{Model}   & {\small{{(All)} $\uparrow$}} & {\small{{(M)} $\uparrow$}} & {\small{{(F)} $\uparrow$}} & \textbf{\small{{GAP} $\downarrow$}} & \textbf{\small{{RMS}} $\downarrow$}\\\midrule
        % \multicolumn{6}{c}{\textit{Occupation Classification - Fine-tuning Setting}} \\ \midrule
        BERT   & 84.14        & 84.69   & 83.50    & 1.189  & 0.144   \\ 
        \midrule
        \textsc{Sent-Debias}  & 83.56       & 84.10   & 82.92   & 1.180  & 0.144   \\
        \textsc{Context-Debias}   & 83.67       & 84.08    & 83.18   & 0.931  & 0.137   \\
        \textsc{FairFil} &  83.18        & 83.52    & 82.78   & 0.746   & 0.142  \\
        \textsc{Adept} &  84.07  & 83.64    & 84.58   & 0.945   &{0.121} \\ 
        \midrule
        \textsc{Mable} &  {84.85}     & {84.92} & {84.34}   & {0.599} & 0.132 \\ 
        \textsc{Mable+$(\mathcal{U}) \mathcal{N C}_3$} &  84.30   & {84.09} & {84.54}   & \bf{0.455} & \bf{0.126} \\
        % \textsc{Mable+$\mathcal{N C}$} &  84.67   & {84.21} & \bf{85.19}   & {0.982} & \bf{0.121} \\ 
        % \midrule
        % \textsc{Adept} &  84.07  & 83.64    & 84.58   & 0.945   & 0.121 \\ 
        % \textsc{Adept+Nc3} &  83.81    & 83.43    & 84.25   & 0.827   & 0.130 \\ 
        \midrule
        \textsc{Ase} &  {84.63}     & {84.19} & {85.14}   & {0.949} & 0.127 \\ 
        \textsc{Ase+$(\mathcal{U}) \mathcal{N C}_3$} &  84.55     & {84.21} & {84.95}   & \bf{0.740} & \bf{0.126} \\ 
        % \textsc{Ase+$\mathcal{N C}$} &  84.62   & \bf{84.27} & {85.02}   & {0.746} & \bf{0.123} \\ 
        \midrule
        \textsc{Bec} &  84.43     & {83.99} & 84.95   & 0.954 & \bf{0.124} \\ 
        \textsc{Bec+$(\mathcal{U}) \mathcal{N C}_3$} &  {84.66}  & {84.23} & {85.17}   & \bf{0.938} & {0.128} \\ 
        % \textsc{Bec+$\mathcal{N C}$} &  {84.59}  & {84.20} & {85.07}   & \bf{0.846} & \bf{0.119} \\ 
        \bottomrule
        \end{tabular}
        }
        \label{tab:occ-cls}
    \end{minipage}
    \hfill % This will push the tables apart to fill the line
    \begin{minipage}[b]{0.48\textwidth}
        \centering
        \caption{Results on Bias-NLI. We fine-tune the models on SNLI and then evaluate on Bias-NLI.}
        \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{lcccc} \toprule
              \textbf{Model} & \textbf{NN} $\uparrow$ & \textbf{FN} $\uparrow$ & \textbf{T:0.5} $\uparrow$ & \textbf{T:0.7}  $\uparrow$ \\ \midrule
        \textsc{BERT}                 & 0.799 & 0.879 & 0.874 & 0.798\\
        \midrule
        \textsc{Sent-Debias}               & 0.793 & 0.911 & 0.897 & 0.788 \\
        \textsc{Context-Debias}             & 0.858 & 0.906 & 0.902 & 0.857 \\
        \textsc{FairFil}               & 0.829 & 0.883 & 0.846 & 0.845 \\ 
        \textsc{Adept}  & 0.841 & 0.937 & 0.934 & 0.866\\
        \midrule
        \textsc{Mable} & \bf{0.900} & {0.977} & {0.974} & \bf{0.935}\\
        \textsc{Mable+$(\mathcal{U}) \mathcal{N C}_3$} & {0.882} & {0.977} & {0.974} & {0.919}\\
        % \textsc{Mable+$\mathcal{N C}$} & {0.873} & {0.973} & {0.970} & {0.904}\\
        % \midrule
        % \textsc{Adept}  & 0.841 & 0.937 & 0.934 & 0.866\\
        % \textsc{Adept+Nc3} & 0.877 & 0.930 & 0.929 & 0.881\\
        \midrule
        \textsc{Ase} & 0.886 & 0.974 & 0.971 & 0.932 \\
        \textsc{Ase+$(\mathcal{U}) \mathcal{N C}_3$} & \bf{0.910}  & 0.974  & \bf{0.973} & \bf{0.948}\\
        % \textsc{Ase+$\mathcal{N C}$} & {0.902} & {0.961} & {0.959} & {0.925}\\
        \midrule
        \textsc{Bec} & \bf{0.933} & 0.955 & 0.955 & 0.934 \\
        \textsc{Bec+$(\mathcal{U}) \mathcal{N C}_3$} & {0.883}  & \bf{0.980}  & \bf{0.978} & \bf{0.943}\\
        % \textsc{Bec+$\mathcal{N C}$} & {0.878} & \bf{0.983} & \bf{0.980} & {0.929}\\
        \bottomrule
        \end{tabular}
        }
        \label{tab:nli}
    \end{minipage}
\end{table}
